Is your benchmark truly adversarial? AdvScore: Evaluating Human-Grounded Adversarialness

Adversarial datasets should validate AI robustness by providing samples on which humans perform well, but models do not. However, as models evolve, datasets can become obsolete. Measuring whether a dataset remains adversarial is hindered by the lack of a standardized metric for measuring adversarialness. We propose AdvScore, a human-grounded evaluation metric that assesses a dataset's adversarialness by capturing models' and humans' varying abilities while also identifying poor examples. We then use AdvScore to motivate a new dataset creation pipeline for realistic and high-quality adversarial samples, enabling us to collect an adversarial question answering (QA) dataset, AdvQA. We apply AdvScore using 9,347 human responses and ten language models' predictions to track model improvement over five years, from 2020 to 2024. AdvScore thus provides guidance for achieving robustness comparable with human capabilities. Furthermore, it helps determine to what extent adversarial datasets continue to pose challenges, ensuring that, rather than reflecting outdated or overly artificial difficulties, they effectively test model capabilities.

==> sections/110-retracingDADC.tex <==
% \section{Retracing DADC for \abr{llms}} \label{retracellms}

% % To test this, introduce interface that includes llms and retrieval model 
% To investigate if and how \abr{llm}s impact the adversarial writing process in \abr{DADC} setting, we present an interactive adversarial question
% generation interface \textit{updated} with retrieval models and powerful \abr{llms} (Figure~\ref{fig:interface}).
% %
% Unlike the traditional \abr{DADC} interface, we include a component that simultaneously
% displays predictions of \abr{llm}-powered \abr{qa} models. Moreover, to combat the opaqueness of \abr{llm}s, we demonstrate different types of retrieval models that yield evidence where the model attained hints for prediction; this way, writers can reason why their questions failed to stump the model and tweak initially written questions (\S\ref{interface}). 
% %
% Through our interactions with users, we discovered that \abr{llm}s also encouraged a new failure mode of adversarial questions: overly vague questions that neither humans nor computers could answer (Figure~\ref{fig:diagram}). 
% %
% These vague questions aligned with errors in current \abr{qa} datasets:
% ambiguity~\citep{min2020ambigqa}, contain false presuppositions~\citep{min2022crepe} or questionable
% assumptions~\cite{kim20222}.  
% We had a significantly higher proportion of usable questions when the authors were trained to write good questions for humans.

==> sections/115-aretheygoodquestions.tex <==
% \section{Results: Are they Good Questions?} \label{aretheygood}
% %
% This section evaluates and analyzes the questions written in the interface
% designed to target \abr{llm}-powered \abr{qa} models (e.g., T5 and
% DistilBert); we explore 1) the question quality with our incentive metric 2)
% what kind of adversarial techniques appear in \textit{good} and \textit{poor}
% questions 3) how questions that stump the \abr{llm}s in the interface
% generalize when applied to more complex \abr{llm}s (e.g., \abr{chatgpt}), and
% 4) how explanations from retrieval models help in constructing an adversarial
% proxy to stump the \abr{llm}s. To make this feasible, we hold two rounds of
% competition with 12 author teams and 12 answerer (human and machine) teams. In
% answerer teams, there were eight human teams\footnote{The authors and human
%   teams were formed by volunteers from the Trivia Community and college students.} and four machine
% answerers (e.g., \abr{dpr}, \abr{t5}, \abr{distilbert}, and \abr{chatgpt}).
% %

% We noticed that there was an improvement in question quality when authored by
% Trivia writers acquainted with ``trivia
% norms''~\citep{boyd-graber-borschinger-2020-question,
%   rodriguez2021evaluation}. The question sets written by Trivia experts
% contained 57\% acceptable questions, while those written by college
% students contained 38\%. One failure mode of vague questions was \enquote{What video game movie featuring one of the \textit{most  popular} and \textit{well-known} icons in video games stars Chris Pratt and Jack Black?}; the question was too subjective.

% %and \enquote{This poet’s most \text{famous} work was mentioned in a television show that tells a story about the people in a women’s prison.}; 
% %
% \subsection{Questions written against \abr{llms}}
% \paragraph{Difficulty}
% To check the adversarial-ness of our questions, we assess how the collected
% questions have a high margin between human difficulty and machine
% difficulty. Table \ref{tab:adversary_raw} demonstrates the number of questions
% that stumped the human and machine teams. The number of questions that stumped \textit{some} humans and \textit{all} machines were the highest. Also, the ratio of correctly answering the
% questions from the most competent human team to the computer team was 79 to
% 21, suggesting that most of the questions were adversarial.
% \begin{table}[!h]
%     \renewcommand{\arraystretch}{1.2}
%     \setlength{\tabcolsep}{2pt}
%     \centering
%     \small
%     \begin{tabular}{cccc}
%     \Xhline{1pt}
%         & \multicolumn{2}{c}{Number of Questions Stumped} \\
%     \Xhline{1pt}
%     && \multicolumn{2}{c}{\quad \quad \quad \abr{Machine}}\\
%           \multirow{-2}{*}{} &&{All} & {Some} \\ 
%          \Xhline{1pt}
%          \multirow{2}{*}{\abr{Human}}& {\quad \quad All}   &  73     & 8 \\
%          & {\quad \quad Some} &  \textbf{90}    & 13 \\
%     \Xhline{1pt}
%     \end{tabular}
%     \caption{The number of questions that stumped \textit{some} humans and
%       \textit{all} machines were the highest: 90 adversarial questions.}
%     \label{tab:adversary_raw}
% \end{table}
% \noindent
% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=\linewidth]{figures/human_machine_difficulty.pdf}
%     \caption{The number of questions that \entoure[red]{stump only machines} (top left) was comparable with the number of questions that \entoure[blue]{stump both} \entoure[blue]{humans and machines} (top right).} 
%     \label{fig:human_machine difficulty}
% \end{figure}
% \noindent

% Figure \ref{fig:human_machine difficulty} shows four clusters of questions
% according to the $\theta_j^{(h)}$ and $\theta_j^{(c)}$ learned from the IRT
% models. The red cluster (top left) denotes the questions that
% \entoure[red]{stump only the machines} ($39\%$), the blue cluster (top right)
% denotes the questions that \entoure[blue]{stump both humans and machines}
% ($36\%$), the black cluster (bottom right) denotes the questions that
% \entoure[black]{stump only the humans} ($13\%$), and green cluster (bottom
% left) denotes the questions that are \entoure[green]{easy} ($11\%$). We infer
% that our framework helps create adversarial questions\footnote{The questions
%   that stumped both do not necessarily mean that they are not
%   adversarial. These questions may not be as easy as the writers intended them
%   when writing, as writers and answerers may have different knowledge or
%   answering skills.}. Table~\ref{table:humanmachinedifficultyexample}
% illustrates the examples that have the highest margin between human difficulty
% and machine difficulty per cluster.

% \begin{table}[!h]
%     \centering
%     \small
%     \setlength{\tabcolsep}{8pt} 
%     \renewcommand{\arraystretch}{1.6}
%     \begin{tabular}{p{15mm}p{35mm}p{11mm}}
%     \Xhline{1pt}
%          \textbf{Stumped Subjects} & \quad \quad \quad \textbf{Question} & \textbf{Answer}\\ 
%     \Xhline{1pt}
%         \entoure[red]{Only} \quad \quad \entoure[red]{Machines}  &  {A German admiral sailing for Russia named what islands for an English captain and not for the librettist of the HMS Pinafore nor for the announcer of Jeopardy!}  & Gilbert Islands    \\
%         %
%         \entoure[blue]{Machines} \quad \quad \entoure[blue]{and Humans}  & {What color did Real Madrid wear during the 2017 Champions League final?}  & Purple  \\
%         %
%         \entoure[black]{Only Humans}  & {Which of the first Adidas Yeezy Boost 350 designs had an out of this world themed name?} & Moonrock  \\
%         %
%         \entoure[green]{Easy}  & {What famous art piece that is currently in France is referred to as La Giaconda?} & Mona Lisa  \\
%         \Xhline{1pt}
%     \end{tabular}
%     \caption{From each cluster, we display examples that had the highest margin between the human and machine difficulty.}
%     \label{table:humanmachinedifficultyexample}
% \end{table}

% \paragraph{Discriminability}
% Also, we check the discriminability value ($\gamma$) of the collected questions. Table~\ref{table:disc_example} shows the questions sorted by $\gamma$. The questions with the highest values were only answered by teams familiar with literature and history; the adversarial tactic of \textit{Domain \& Commonsense knowledge} was used so that the question could be only answered by models trained on specific knowledge. Moreover, high discriminability data points are scattered across all difficulty levels, meaning that questions at all difficulty levels mostly rewarded the answerer's skill (Figure~\ref{fig:diagram}). 

% \begin{table}[!h]
%     \centering
%     \small
%     \setlength{\tabcolsep}{8pt} 
%     \renewcommand{\arraystretch}{1.6}
%     \begin{tabular}{p{40mm}p{15mm}p{5mm}}
%     \Xhline{1pt}
%          \qquad\qquad\textbf{Question} & \textbf{Answer} & \textbf{$\gamma$} \\
%     \Xhline{1pt}
%         {What city in England is home to the studios where the British game show that resembles quiz bowl is filmed and where the test of whether an AI is intelligent was proposed?}  &  Manchester & {0.193} \\
%         {The 1973 Thomas Rockwell novel for children, about a school boy who loses a gross dare, was written in America. However, a similarly-titled religious edict published in 1521 hails from this old European city of about 80,000.}  &  Worms, Germany & {0.192} \\
%         \qquad\qquad\qquad\qquad\qquad\qquad\qquad\vdots & \vdots & \vdots \\
%         {Who was able to turn men into stone sculptures by just taking a glance at them?}  &  Medusa & {0.003} \\
%         {Which political party governs the country directly south of Botswana?}  &  African National Congress & {0.003} \\
%         \Xhline{1pt}
%     \end{tabular}
%     \caption{Questions sorted by discriminability($\gamma$) value of the \abr{irt} model.}
%     \label{table:disc_example}
% \end{table}
% %On the other hand, the overlapping negative discriminability and difficulty points indicate that there are some annotation errors \citep{rodriguez-etal-2021-evaluation}. 
 
% \subsection{What kind of adversarial tactics do \abr{llm}s invoke and what makes these less \textit{good}?}
% % AdvType & QType annotation and their examples  
% For a deeper analysis, we scrutinize what kind of adversarial tactics were used by writers to stump \abr{llm}s and evaluate if they are good or poor. To understand \textit{how} they are poor, we examine if there exists any correlation between discriminability and the adversarial tactics the question used.

% We manually tag the questions with problematic question types and adversarial
% types. We added more adversarial types to \citet{wallace2019trick}, such as
% \textit{Domain Expert Knowledge}, and added \textit{Subjectivity} to
% \citet{boyd-graber-borschinger-2020-question} (Appendix~\ref{app:questiontype}
% and \ref{app:advtype}).
% Consider the question \enquote{What is the piece of clothing worn underneath the shirt?}; in some cultures, ``undershirt'' would be the correct answer, while ``pants'' 
% is acceptable for others. In this case, the question type is \textit{subjectivity} and \textit{Lacks specificity}. 
% Likewise, a single question can be poor in different
% ways (examples in Appendix~\ref{app:annotation}).
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/adv_discriminability_pattern.pdf}
%      \caption{The adversarial techniques \textit{Temporal Misalignment}, \textit{Composing Seen Clues}, \textit{Domain Expert Knowledge}, and \textit{Novel Clues} are used more frequently in questions with high discriminability.}
%      \label{fig:adv_disc}
% \end{figure}

% % Quantify adversarial types in Discriminability bins
% From these annotations, we investigate the correlation between what kind of adversarial types appear within questions of different levels of
% discriminability. 
% We find that adversarial writing techniques, such as
% \textit{Temporal Misalignment}, \textit{Composing Seen Clues}, \textit{Domain
%   Expert Knowledge}, and \textit{Novel Clues} often appear in questions with
% high discriminability (Figure \ref{fig:adv_disc}). On the other hand,
% \textit{Logic\&Calculation} technique is used in questions of all
% discriminability levels (Appendix \ref{fig:adv_disc_no}).

% %
% \subsection{Are questions written against retrieval models generalize to \abr{llm}s?} \label{retrievalmodelcomparison}

% We then analyze the impact of retrieval models on the written questions and
% examine if these questions stump the \abr{llm}, as our pieces of evidence are not
% created from the \abr{llm}s but retrieval models. We use \abr{chatgpt} as an
% upper bound for questions to stump and to compare retrieval models; 
% \abr{chatgpt} performs the best among other \abr{llm}s (40\% accuracy). To
% better understand if and how retrieval models were utilized during authoring,
% we first compare the accuracy of retrieval models to \abr{chatgpt}. The
% proportion of questions that stumped both retrieval model and \abr{chatgpt}  was the largest ($65\%$), suggesting that authors who targeted retrieval
% models to write their questions also stump the \abr{chatgpt} (Table
% \ref{tab:stumpaccuracy}). Among the questions that stumped both models, the
% accuracy of T5 and Distilbert were $4\%$, and $0\%$, respectively, which also
% hints at T5's support in writing stumping questions.


% \begin{table}[!h]
%     \renewcommand{\arraystretch}{1.2}
%     \centering
%     \small
%     \begin{tabular}{ccccc}
%     \Xhline{1pt}
%     && \multicolumn{2}{c}{\abr{dpr}}\\
%           \multirow{-2}{*}{} &&{Correct} & {Incorrect}
%          \\ 
%          \Xhline{1pt}
%          %\parbox[t]{2mm}{\multirow{2}{*}%{\rotatebox[origin=c]{90}{\textsc{Chat}}}} 
%          %\parbox[t]{2mm}{\multirow{2}{*}%{\rotatebox[origin=c]{90}{ \textsc{GPT}}}} 
%          \multirow{2}{*}{\abr{ChatGPT}}& Correct   &  2\%     & 32\% \\
%          & Incorrect &  1\%    & \textbf{65\%} \\
%     \Xhline{1pt}
%     \end{tabular}
%     \caption{Percentage of questions stumping both \abr{dpr} and \abr{chatgpt}
%       were the highest among all, indicating that the questions that were
%       written with \abr{dpr} guidance often stump \abr{chatgpt}.}
%     \label{tab:stumpaccuracy}
% \end{table}
% %
% \begin{table*}[!t]
% \centering
%     \normalsize
%     \renewcommand{\arraystretch}{1.5}
%     \resizebox{\textwidth}{!}{
%     \scalebox{1.1}{\begin{tabular}{p{40mm}p{30mm}p{50mm}p{50mm}p{50mm}}
%     \Xhline{1pt}
%      \quad\quad \quad  \multirow{2.3}{*}{\textbf{Question}} & \quad\quad \quad  \multirow{2.3}{*}{\textbf{Answer}}& \multicolumn{3}{c}{\textbf{Explanations}} \\ & &
%     \quad \quad \quad \quad \quad\textbf{Baseline} & \quad \quad \quad \quad \quad \quad  \textbf{\abr{dpr}} & \quad \quad \quad \quad \textbf{\abr{chatgpt}} \\[1.1ex] \Xhline{1pt}
%      %
%      What is the name of the American actor who stood up for \colorbox{red!15}{his wife with a "slap that} \colorbox{red!15}{was heard around the} \colorbox{red!15}{world" during a popular} \colorbox{red!15}{awards show?} & Will Smith & \textit{\textbf{Correct Answer: Will Smith}} \newline "Willard Carroll Smith II (born September 25, 1968), also known by his stage name The Fresh Prince, is an American actor, rapper, and producer." & \textit{\textbf{Correct Answer: Will Smith}} \newline \quad At the 2022 Academy Awards ceremony, shortly before winning, Smith faced public backlash for \colorbox{red!15}{slapping and shouting} at Oscar presenter Chris Rock after Rock made a joke referencing Smith's \colorbox{red!15}{wife}, Jada Pinkett Smith. & \textit{\textbf{Incorrect Answer: Brad Pitt}} \newline The incident of Brad Pitt \colorbox{red!15}{standing up for his wife with} \colorbox{red!15}{a slap during a popular awards} show was widely reported in the media and is a well-known event in popular culture. \\
     
%      What is the name of a famous \colorbox{red!15}{surrealist painting} which originally was thought to be inspired by a \colorbox{red!15}{scientific theory} about space-\colorbox{red!15}{time} but was in fact inspired by a soft, surface-ripened, brie-like \colorbox{red!15}{cheese melting in the sun}? & The Persistence of Memory & \textit{\textbf{Correct Answer: The Persistence of Memory}} \newline Another insect that is present in the painting is a fly, which sits on the watch that is next to the orange watch. & \textit{\textbf{Incorrect answer: A Sunday Afternoon on the Island of La Grande Jatte}}  \newline Inspired by optical effects and perception inherent in the color theories of Michel Eugène Chevreul, Ogden Rood and others, Seurat adapted \colorbox{red!15}{this scientific research to his} \colorbox{red!15}{painting}. & \textit{\textbf{Correct Answer: The Persistence of Memory}}\newline I predicted this answer because The Persistence of Memory is one of the most famous \colorbox{red!15}{surrealist paintings} and is often associated with the concept of \colorbox{red!15}{time}. However, it is also known that the painting was inspired by Salvador Dali's observation of a \colorbox{red!15}{melting} Camembert \colorbox{red!15}{cheese in the sun}.\\

% %     \newline
% %     \textcolor{red}{(Baseline Explanation)} \newline
% %     \textit{\textcolor{red}{Correct Answer: Will Smith}} \newline
% %     \textcolor{red}{(DPR Explanation)} \newline
% %     \textcolor{red}{Correct Answer: Will Smith} \newline
%      \\
%      \bottomrule
%     \end{tabular}}}
%     \caption{Example of evidence that \abr{tfidf}, \abr{dpr}, and \abr{chatgpt} provide for their respective answers. The first example shows an example where retrieval models are not stumped but \abr{llm}s are. The explanations show that \abr{dpr} and \abr{chatgpt} are pointing to the right claims to predict their answers, and it seems like the specificity is lacking in the question that induced the \abr{chatgpt} to be stumped. On the other hand, the \abr{dpr} evidence in the second example was close (has several overlapping spans), but is stumped with the multistep reasoning technique. \abr{chatgpt} captures this nuance and correctly answers the question. \textbf{When we added each retrieval model's explanation, \abr{chatgpt} corrected itself} and answered ``Will Smith''.}
%     \label{tab:explanationcomparison_intext} 
% \end{table*}
% %
% \subsection{How do retrieval model evidence help stump \abr{llm}s?}
% % Compare which IR model explanation more stumps ChatGPT

% \textbf{Utility of evidence}
% Following the analysis on how retrieval model-guided questions generalize
% against \abr{llm}s, we  examine the efficacy of retrieval model
% \textit{evidence} when stumping the \abr{llm}. Here, we use \abr{chatgpt}
% as a human proxy to contrast \textit{which} retrieval model's evidence
% helped \abr{chatgpt} to answer~\citep{guo2023close,
%   mondal2023interactiveie}. We examine the answers based on these evidence
% to check if it was successful in stumping
% \abr{chatgpt}~\citep{ma2023query,liu2023reta}.
% %
% For each question, we retrieve evidence from both the baseline retrieval
% model and \abr{dpr}, and prompt \abr{chatgpt}\footnote{We prompt
%   \abr{chatgpt}, \textit{Do you think that the question can be answered using
%     this evidence from Wikipedia. If yes, predict an answer using the evidence
%     in one or two words.}}. The \abr{chatgpt} will return the answer and
% whether the evidence helped it to answer. We assign
% {\fontfamily{qcr}\selectfont(scores)} to the evidence in three rubrics:
% unhelpful evidence + incorrect answer {\fontfamily{qcr}\selectfont(0)},
% helpful evidence + correct answer {\fontfamily{qcr}\selectfont(1)}, and
% helpful evidence + incorrect answer {\fontfamily{qcr}\selectfont(2)}. Score
% {\fontfamily{qcr}\selectfont(2)} indicates that the question with \textit{the
%   evidence} stumped the \abr{chatgpt} model. Then, we averaged the scores
% (baseline retrieval: 0.22, \abr{dpr}: 0.32), finding that \abr{dpr}'s
% evidence is $10\%$ more helpful in writing questions that stumped
% \abr{chatgpt}.

% \noindent
% \textbf{Error Analyses with Evidence} 
% It is reassuring that retrieval-based approaches seem to generalize to "closed-book" models.  We next look at how the evidence generalize from retrieval models to advanced models like ChatGPT and vice versa.\\
% %
% To retrieve \abr{chatgpt} explanation for each question, we prompt\footnote{We
%   prompt ChatGPT, \textit{"Answer the question in one or two words and provide
%     an explanation for your answer."}} it to return an answer and its
% groundings. The comparison examples are demonstrated in
% Table~\ref{tab:explanationcomparison_intext}.
% %
% First, ChatGPT does not provide good explanations of \textit{why} it answers
% something when it was incorrect, suggesting that spurning such models'
% explanations in our interface was wise: it hallucinates ``Brad Pitt'' slapping
% someone at an awards show. But when provided the relevant context from
% retrieval models with access to more up-to-date material, it gets the answer
% correct, a la retrieval-augmented QA systems like
% \citet{siriwardhana2023improving}. This suggests that it would also get the
% correct answer if it were updated. However, ChatGPT gets the answer
% correct when its explanations are similar to more traditional retrieval
% systems, partially explaining the outcome overlap we discovered in Section
% ~\ref{retrievalmodelcomparison} (More examples in
% Appendix~\ref{app:explanationcomparison}).



% % Compare two ir models, chatgpt explanation


% \begin{comment}
%  Figure \ref{fig:groupscore} illustrates the distribution of $Score$ of 8 teams, where the average is $-0.28$, and the standard deviation is $1.72$, where the H team scored the best. One winning question was ``\textit{Name the Kentucky quarterback that against all predictions, was not drafted in the first round of the 2023 NFL draft.}'', which used ``negation'' technique and current event that stumps the model.
% %Todo: (Appendix) more example of best team's questions

% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=\linewidth]{figures/group_score.pdf}
%     \caption{The questions are distributed fairly evenly in perspective of difficulty and discriminability.} 
%     \label{fig:groupscore}
% \end{figure}
% \end{comment}




% %Also, we identify the most and least difficult questions by sorting $\theta$. For example, \textit{``What is the name of the language which only has 45,900 speakers, allows for word-initial double consonants, and is the official language of an island country with the world’s second-largest
% %regional shark sanctuary?''} was ranked the most difficult, while \textit{``Which political party governs the country directly south of Botswana?''} was ranked the least difficult (answers below\footnotetext{\raggedleft\rotatebox{180}{$^1$ Chuukese \qquad $^2$ African National Congress}}).



% %- Diversity Evaluation
% %NER -> country representation -> distribution of questions. 



==> sections/116-datasetcreation.tex <==


% \jbgcomment{Again, I think it's best to structure this as first proving the metric is good with historical data and then getting to our new stuff.}

% Our goal in crafting adversarial questions lies in probing the ability of the
% \abr{QA} models (e.g., is it robust to adversarial attacks?) rather than
% satisfying the users who use \abr{QA} models with information-seeking
% purposes~\citep{rogers2023qa}.
%
% \subsection{\advqa{} Interface}
% \begin{figure*}[!h]
%     \centering
%     \includegraphics[width=0.98\textwidth]{figures/interface.pdf}
%     \caption{As the target answer to the question should be ``Apple Inc,'' the interface is updated with answers from retrieval models with the most relevant sentence and from \abr{lm}s (e.g., Distilbert, T5). Also, the highlights are updated by the input perturbation technique.} 
%     \label{fig:interface}
% \end{figure*}







==> sections/checklist.tex <==
\section*{Checklist}
\begin{enumerate}
% \answerNA{}
% \answerYes{}
% \answerNo{}
\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{} (See \S \ref{conclusion})
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{} (See \S \ref{conclusion})
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them? 
    \answerYes{} (See Appendix \S \ref{Ethics})
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{} (See \S \ref{irt})
	\item Did you include complete proofs of all theoretical results?
    \answerYes{} (See \S \ref{comparison})
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} 
    (We include data, data description \& instructions, and github repository url in the the supplemental material.)
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} (We specify benchmark details in \S \ref{comparison}.)
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{} No (Our metric does not need error bars)
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{} (Our study does not require intensive computing power.)
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} (See \S \ref{comparison})
  \item Did you mention the license of the assets?
    \answerYes{} (Some of them did not have license)
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes (We include the existing and curated, new assets in the supplemental material)
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{} (We include the consent forms used in our user study and related IRB forms in the supplementary material.)
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{} (Additionally, this work is approved by official IRB board. See Appendix \ref{Ethics}.)
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{} (We include instructions for our user study in the supplementary material and provided interface screenshot in Appendix~\ref{interface_screenshot} )
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerYes{} (We include such information in the consent forms and \S \ref{Ethics})
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{} (Our study was based on prizes; we include prize details in the supplemental material and footnote in p.6)
\end{enumerate}

\end{enumerate}
